Detecting train driveshaft damages using accelerometer signals and Differential Convolutional Neural Networks

Railway axle maintenance is critical to avoid catastrophic failures. Nowadays, condition monitoring techniques are becoming more prominent in the industry to prevent enormous costs and damage to human lives. This paper proposes the development of a railway axle condition monitoring system based on advanced 2D-Convolutional Neural Network (CNN) architectures applied to time-frequency representations of vibration signals. For this purpose, several preprocessing steps and different types of Deep Learning (DL) and Machine Learning (ML) architectures are discussed to design an accurate classification system. The resultant system converts the railway axle vibration signals into time-frequency domain representations, i.e., spectrograms, and, thus, trains a two-dimensional CNN to classify them depending on their cracks. The results showed that the proposed approach outperforms several alternative methods tested. The CNN architecture has been tested in 3 different wheelset assemblies, achieving AUC scores of 0.93, 0.86, and 0.75 outperforming any other architecture and showing a high level of reliability when classifying 4 different levels of defects.

==> formulas.tex <==
\newcommand{\method}{SSHIBA } %method name
\newcommand{\R}{\mathbb{R}} %Real numbers
\newcommand{\Na}{\mathbb{N}} %Real numbers
\newcommand{\E}{\mathbb{E}} %Expectation
\newcommand{\N}{\mathcal{N}} %gaussian normal
\newcommand{\W}{\mathcal{W}} %wishart
\newcommand{\M}{\mathcal{M}} %Conjunto
\newcommand{\const}{\text{const}} %Expectation
\DeclareMathOperator{\Tr}{Tr} %Traze operator
\DeclareMathOperator*{\argmin}{argmin} %argmin operator
\DeclareMathOperator*{\argmax}{argmax} %argmax operator

% Parenthesis \left( \right) automatically
% Normal parentheses: \p{1+2}

% Left-right parentheses: \p*{1+2}
% Sized-control parentheses: \p[\Big]{1+2}

% ****************************** Variables definition ***************************** %
\DeclareMathOperator{\X}{\mathbf{X}} %X
\DeclareMathOperator{\Xo}{\mathbf{Z}^{(O)}} %X^(m)
\DeclareMathOperator{\Xon}{\mathbf{z}_{n,:}^{(O)}} %X^(m)
\DeclareMathOperator{\Xonp}{\mathbf{z}_{n,:}^{*(O)}} %X^(m)
\DeclareMathOperator{\Xa}{\mathbf{Z}^{(A)}} %X^(m)
\DeclareMathOperator{\Xan}{\mathbf{z}_{n,:}^{(A)}} %X^(m)
\DeclareMathOperator{\xC}{\mathbf{z}^{(C)}} %X^(m)
\DeclareMathOperator{\XC}{\mathbf{Z}^{(C)}} %X^(m)
\DeclareMathOperator{\XD}{\mathbf{Z}^{(D)}} %X^(m)
\DeclareMathOperator{\xD}{\mathbf{z}^{(D)}} %X^(m)
\DeclareMathOperator{\Xm}{\mathbf{Z}^{(m)}} %X^(m)
\DeclareMathOperator{\Xmt}{\mathbf{Z}^{\{\M_t\}}} %X^(m)
\DeclareMathOperator{\Xmmt}{\mathbf{Z}^{(m_t)}} %X^(m)
\DeclareMathOperator{\xnmmt}{\mathbf{x}^{(m_t)}_{n,:}} %X^(m)
\DeclareMathOperator{\XM}{\mathbf{X}^{M}} %X^(M)
\DeclareMathOperator{\Xone}{\mathbf{X}^{(1)}} %X^(1)
\DeclareMathOperator{\Xtwo}{\mathbf{X}^{(2)}} %X^(2)
\DeclareMathOperator{\XmT}{\mathbf{Z}^{(m)^T}} %X^(m)^T
\DeclareMathOperator{\XoneT}{\mathbf{X}^{(1)^T}} %X^(1)^T
\DeclareMathOperator{\XtwoT}{\mathbf{X}^{(2)^T}} %X^(2)^T
\DeclareMathOperator{\Xnm}{\mathbf{x}_{n,:}^{(m)}} %X_n^(m)
\DeclareMathOperator{\Fnm}{\mathbf{z}_{n,:}^{(m)}} %X_n^(m)
\DeclareMathOperator{\Fm}{\mathbf{z}^{(m)}} %X_n^(m)
\DeclareMathOperator{\Inm}{\mathbf{i}_{n,:}^{(m)}} %X_n^(m)
\DeclareMathOperator{\Onmr}{\mathbf{\Tilde{x}}_{n,:}^{(m)}} %*O_n^(m)
\DeclareMathOperator{\Onm}{\mathbf{x}_{n,:}^{(m)}} %O_n^(m)
\DeclareMathOperator{\Om}{\mathbf{X}} %O_(m)
\DeclareMathOperator{\On}{\mathbf{X}_{n}} %O_(m)
\DeclareMathOperator{\XnmD}{\mathbf{x}_{n,1}^{(m)}} %X_n^(m)
\DeclareMathOperator{\Xonem}{\mathbf{x}_{1,:}^{(m)}} %X_1^(m)
\DeclareMathOperator{\XNm}{\mathbf{x}_{N,:}^{(m)}} %X_N^(m)
\DeclareMathOperator{\XnMlast}{\mathbf{x}_{n,:}^{(M)}} %X_n^(m)
\DeclareMathOperator{\XnM}{\mathbf{x}_{n,:}^{\{\M\}}} %X_n^(m)
\DeclareMathOperator{\Xnmt}{\mathbf{x}_{n,:}^{\{\M_t\}}} %X_n^(m)
\DeclareMathOperator{\Xnone}{\mathbf{x}_{n,:}^{(1)}} %X_n^(1)
\DeclareMathOperator{\Xntwo}{\mathbf{x}_{n,:}^{(2)}} %X_n^(2)
\DeclareMathOperator{\Xndottwo}{\mathbf{x}_{n,:}^{(2)}} %X_{n:}^(2)
\DeclareMathOperator{\XnmT}{\mathbf{x}_{n,:}^{(m)^T}} %X_n^(m)^T
\DeclareMathOperator{\XnoneT}{\mathbf{x}_{n,:}^{(1)^T}} %X_n^(1)^T
\DeclareMathOperator{\XntwoT}{\mathbf{x}_{n,:}^{(2)^T}} %X_n^(2)^T
\DeclareMathOperator{\Xndm}{x_{n,d}^{(m)}} %X_nd^(m)
\DeclareMathOperator{\XndD}{x_{n,1}^{(D)}}
\DeclareMathOperator{\XndT}{x_{n,d}^{(T)}}
\DeclareMathOperator{\Xndone}{x_{n,d}^{(1)}} %X_nd^(1)
\DeclareMathOperator{\Xndtwo}{x_{n,d}^{(2)}} %X_nd^(2)
\DeclareMathOperator{\Xnim}{x_{n,i}^{(m)}} %X_ni^(m)
\DeclareMathOperator{\Xnimt}{x_{n,i}^{(m_t)}} %X_ni^(m)
\DeclareMathOperator{\Xnione}{x_{n,i}^{(1)}} %X_ni^(1)
\DeclareMathOperator{\Xnitwo}{x_{n,i}^{(2)}} %X_ni^(2)
\DeclareMathOperator{\Xnjm}{x_{n,j}^{(m)}} %X_nj^(m)
\DeclareMathOperator{\Xnjmt}{x_{n,j}^{(m_t)}} %X_nj^(m)
\DeclareMathOperator{\Xnjone}{x_{n,j}^{(1)}} %X_nj^(1)
\DeclareMathOperator{\Xnjtwo}{x_{n,j}^{(2)}} %X_nj^(2)
\DeclareMathOperator{\XndmT}{x_{n,d}^{(m)^T}} %X_nd^(m)^T
\DeclareMathOperator{\XndoneT}{x_{n,d}^{(m)^T}} %X_nd^(1)^T
\DeclareMathOperator{\XndtwoT}{x_{n,d}^{(2)^T}} %X_nd^(2)^T
\DeclareMathOperator{\Xdm}{\mathbf{x}_{:,d}^{(m)}} %X_:d^(m)
\DeclareMathOperator{\XdmT}{\mathbf{x}_{:,d}^{(m)^T}} %X_:d^(m)^T
\DeclareMathOperator{\XdoneT}{\mathbf{x}_{:,d}^{(1)^T}} %X_:d^(1)^T
\DeclareMathOperator{\XdtwoT}{\mathbf{x}_{:,d}^{(2)^T}} %X_:d^(2)^T
\DeclareMathOperator{\xndmtwo}{x_{n,d}^{(m)^2}}

\DeclareMathOperator{\XmS}{\mathbf{\tilde{X}}^{(m)}} %X^(m)*
\DeclareMathOperator{\XmoutS}{\mathbf{\tilde{X}}^{\{\M_{out}\}}} %X^(m)*
\DeclareMathOperator{\xnmoutS}{\mathbf{x}^{\{\M_{out}\}}_{new,:}} %X^(m)*
\DeclareMathOperator{\xnminS}{\mathbf{x}^{\{\M_{in}\}}_{new,:}} %X^(m)*
\DeclareMathOperator{\XminS}{\mathbf{\tilde{X}}^{\{\M_{in}\}}} %X^(m)*
\DeclareMathOperator{\XoneS}{\mathbf{\tilde{X}}^{(1)}} %X^(1)*
\DeclareMathOperator{\XtwoS}{\mathbf{\tilde{X}}^{(2)}} %X^(2)*
\DeclareMathOperator{\XdmS}{\mathbf{\tilde{X}}_{:,d}^{(m)}} %X_d^(m)*
\DeclareMathOperator{\XnmS}{\mathbf{x}_{new,:}^{(m)}} %X_n^(m)*
\DeclareMathOperator{\XnoneS}{\mathbf{\tilde{x}}_{n,:}^{(1)}} %X_n^(1)*
\DeclareMathOperator{\XntwoS}{\mathbf{\tilde{x}}_{n,:}^{(2)}} %X_n^(2)*
\DeclareMathOperator{\XndmS}{\tilde{x}_{n,d}^{(m)}} %X_nd^(m)*
\DeclareMathOperator{\XndminS}{\tilde{x}_{n,d}^{\{\M_{in}\}}} %X_nd^(m_in)*
\DeclareMathOperator{\XndmoutS}{x_{new,d}^{\{\M_{out}\}}} %X_nd^(m_out)*
\DeclareMathOperator{\XdmoutS}{\mathbf{x}_{:,d}^{\{\M_{out}\}}} %X_d^(m_out)*
\DeclareMathOperator{\XndoneS}{\tilde{x}_{n,d}^{(1)}} %X_nd^(1)*
\DeclareMathOperator{\XndtwoS}{\tilde{x}_{n,d}^{(2)}} %X_nd^(2)*
\DeclareMathOperator{\XnimS}{\tilde{x}_{n,i}^{(m)}} %X_ni^(m)*
\DeclareMathOperator{\xnimoutS}{x_{new,i}^{\{\M_{out}\}}} %X_ni^(m)*
\DeclareMathOperator{\XnioneS}{\tilde{x}_{n,i}^{(1)}} %X_ni^(1)*
\DeclareMathOperator{\XnitwoS}{\tilde{x}_{n,i}^{(2)}} %X_ni^(2)*
\DeclareMathOperator{\XnjmS}{\tilde{x}_{nj}^{(m)}} %X_nj^(m)*
\DeclareMathOperator{\XnjoneS}{\tilde{x}_{nj}^{(1)}} %X_nj^(1)*
\DeclareMathOperator{\XnjtwoS}{\tilde{x}_{nj}^{(2)}} %X_nj^(2)*
\DeclareMathOperator{\xndminS}{x_{new,d}^{\{\M_{in}\}}}
\DeclareMathOperator{\xndmoutS}{x_{new,d}^{\{\M_{out}\}}}
\DeclareMathOperator{\xndrS}{\tilde{x}_{n,d}^{\{\M_{r}\}}}
\DeclareMathOperator{\XndrS}{\tilde{x}_{n,d}^{\{\M_{r}\}}}
\DeclareMathOperator{\xdrS}{\mathbf{\tilde{x}}_{:,d}^{\{\M_{r}\}}}
\DeclareMathOperator{\xndtS}{\tilde{x}_{n,d}^{\{\M_{t}\}}}
\DeclareMathOperator{\XndtS}{\tilde{x}_{n,d}^{\{\M_{t}\}}}
\DeclareMathOperator{\XdtS}{\mathbf{\tilde{x}}_{:,d}^{\{\M_{t}\}}}

\DeclareMathOperator{\Km}{\mathbf{K}^{(m)}}
\DeclareMathOperator{\Kone}{\mathbf{K}}
\DeclareMathOperator{\KmT}{\mathbf{K}^{(m)^T}}
\DeclareMathOperator{\Knone}{\mathbf{k}_{n,:}}
\DeclareMathOperator{\Knm}{\mathbf{k}_{n,:}^{(m)}}
\DeclareMathOperator{\Ksnm}{\mathbf{\tilde{k}}_{n,:}^{(m)}}
\DeclareMathOperator{\KnmT}{\mathbf{k}_{n,:}^{(m)^T}}
\DeclareMathOperator{\Knsm}{\mathbf{k}_{:,n^{*}}^{(m)}}
\DeclareMathOperator{\KnsmT}{\mathbf{k}_{:,n^{*}}^{(m)^T}}
% \DeclareMathOperator{\Knnsm}{k_{n,\tilde{n}}^{(m)}}
\DeclareMathOperator{\Knnsm}{k_{n,n}^{(m)}}
\DeclareMathOperator{\Knum}{k_{n,u}^{(m)}}
\DeclareMathOperator{\Kum}{\mathbf{k}_{:,u}^{(m)^T}}
\DeclareMathOperator{\KumT}{\mathbf{k}_{:,u}^{(m)^T}}
\DeclareMathOperator{\KM}{\mathbf{K}^{\{\M\}}} %X^(M)
\DeclareMathOperator{\KnM}{\mathbf{k_{n,:}}^{\{\M\}}} %X^(M)

\DeclareMathOperator{\Lm}{\text{\boldmath$\Lambda$}^{(m)}} %X^(M)
\DeclareMathOperator{\lm}{\text{\boldmath$\lambda$}^{(m)}} %X^(M)
\DeclareMathOperator{\lmnew}{\text{\boldmath$\lambda$}_{new}^{(m)}} %X^(M)
\DeclareMathOperator{\lmold}{\text{\boldmath$\lambda$}_{old}^{(m)}} %X^(M)
\DeclareMathOperator{\lonem}{\lambda_1^{(m)}} %X^(M)
\DeclareMathOperator{\lDm}{\lambda_{D_m}^{(m)}} %X^(M)
\DeclareMathOperator{\ldm}{\lambda_d^{(m)}} %X^(M)

\DeclareMathOperator{\Rm}{\mathbf{R}^{(m)}}
\DeclareMathOperator{\Rnsnsm}{\mathbf{r}_{n^{*},n^{*}}^{(m)}}

\DeclareMathOperator{\ynm}{\mathbf{y}_{n,:}^{(m)}}
\DeclareMathOperator{\ynmt}{\mathbf{y}_{n,:}^{(m_t)}}
\DeclareMathOperator{\ynim}{\mathbf{y}_{n,i}^{(m)}}
\DeclareMathOperator{\ynimt}{\mathbf{y}_{n,i}^{(m_t)}}
\DeclareMathOperator{\ynjm}{\mathbf{y}_{n,j}^{(m)}}
\DeclareMathOperator{\ynjmt}{\mathbf{y}_{n,j}^{(m_t)}}
\DeclareMathOperator{\ynkmt}{\mathbf{y}_{n,k}^{(m_t)}}

\DeclareMathOperator{\Z}{\mathbf{G}} %Y
\DeclareMathOperator{\Zp}{\mathbf{g}_{n,:}^*} %Zpredict
\DeclareMathOperator{\ZS}{\mathbf{\tilde{G}}} %Y^*
\DeclareMathOperator{\ZT}{\mathbf{G}^T} %Y^T
\DeclareMathOperator{\ZST}{\mathbf{\tilde{G}}^{T}} %Y^T^*
\DeclareMathOperator{\Zn}{\mathbf{g}_{n,:}} %Y
\DeclareMathOperator{\ZnS}{\mathbf{\tilde{g}}_{n,:}} %Y^*
\DeclareMathOperator{\ZnT}{\mathbf{g}_{n,:}^T} %Y^T
\DeclareMathOperator{\ZnST}{\mathbf{\tilde{g}}_{n,:}^{T}} %Y^*^T
\DeclareMathOperator{\znS}{\tilde{g}_n} %z_n^*

\DeclareMathOperator{\zS}{\mathbf{g}_{new,:}} %z^*

\DeclareMathOperator{\Am}{\mathbf{A}^{(m)}} %\mathbf{w}_:k^(m)
\DeclareMathOperator{\Aone}{\mathbf{A}} %\mathbf{w}_:k^(m)
\DeclareMathOperator{\AoneT}{\mathbf{A}^T} %\mathbf{w}_:k^(m)
\DeclareMathOperator{\AmT}{\mathbf{A}^{(m)^T}} %\mathbf{w}_:k^(m)
\DeclareMathOperator{\Akm}{\mathbf{a}_{:,k}^{(m)}} %\mathbf{w}_:k^(m)
\DeclareMathOperator{\AkmT}{\mathbf{a}_{:,k}^{(m)^T}} %\mathbf{w}_:k^(m)
\DeclareMathOperator{\Anm}{\mathbf{a}_{n,:}^{(m)}} %\mathbf{w}_:k^(m)
\DeclareMathOperator{\Ansm}{\mathbf{a}_{\tilde{n},:}^{(m)}} %\mathbf{w}_:k^(m)
\DeclareMathOperator{\Aum}{\mathbf{a}_{u,:}^{(m)}} %\mathbf{w}_:k^(m)
% % \DeclareMathOperator{\Ansm}{\mathbf{a}_{n,:}^{(m)}} %\mathbf{w}_:k^(m)
\DeclareMathOperator{\AnsmT}{\mathbf{a}_{\tilde{n},:}^{(m)^T}} %\mathbf{w}_:k^(m)
\DeclareMathOperator{\AumT}{\mathbf{a}_{u,:}^{(m)^T}} %\mathbf{w}_:k^(m)
% % \DeclareMathOperator{\AnsmT}{\mathbf{a}_{n,:}^{(m)^T}} %\mathbf{w}_:k^(m)
\DeclareMathOperator{\Anskm}{a_{\tilde{n},k}^{(m)}} %\mathbf{w}_:k^(m)
\DeclareMathOperator{\Aukm}{a_{u,k}^{(m)}} %\mathbf{w}_:k^(m)
% \DeclareMathOperator{\Anskm}{a_{n,k}^{(m)}} %\mathbf{w}_:k^(m)
\DeclareMathOperator{\Ankm}{a_{n,k}^{(m)}} %\mathbf{w}_:k^(m)

\DeclareMathOperator{\Wo}{\mathbf{W}^{(O)}} %W^(o)
\DeclareMathOperator{\Wa}{\mathbf{W}^{(A)}} %W^(a)
\DeclareMathOperator{\WD}{\mathbf{W}^{(D)}} %W^(D)
\DeclareMathOperator{\Wm}{\mathbf{W}^{(m)}} %W^(m)
\DeclareMathOperator{\Wmout}{\mathbf{W}^{\{\M_{out}\}}} %W^(m)
\DeclareMathOperator{\Wone}{\mathbf{W}^{(1)}} %W^(1)
\DeclareMathOperator{\Wtwo}{\mathbf{W}^{(2)}} %W^(2)
\DeclareMathOperator{\WaT}{\mathbf{W}^{(A)^T}} %W^(m)^T
\DeclareMathOperator{\WoT}{\mathbf{W}^{(O)^T}} %W^(m)^T
\DeclareMathOperator{\WmT}{\mathbf{W}^{(m)^T}} %W^(m)^T
\DeclareMathOperator{\WmtT}{\mathbf{W}^{\{\M_t\}^T}} %W^(m)^T
\DeclareMathOperator{\WmmtT}{\mathbf{W}^{(m_t)^T}} %W^(m)^T
\DeclareMathOperator{\WmoutT}{\mathbf{W}^{\{\M_{out}\}^T}} %W^(m)^T
\DeclareMathOperator{\WoneT}{\mathbf{W}^{(1)^T}} %W^(1)^T
\DeclareMathOperator{\WtwoT}{\mathbf{W}^{(2)^T}} %W^(2)^T
\DeclareMathOperator{\Wkm}{\mathbf{w}_{:,k}^{(m)}} %\mathbf{w}_:k^(m)
\DeclareMathOperator{\Wkone}{\mathbf{w}_{:,k}^{(1)}} %\mathbf{w}_:k^(1)
\DeclareMathOperator{\Wktwo}{\mathbf{w}_{:,k}^{(2)}} %\mathbf{w}_:k^(2)
\DeclareMathOperator{\WkmT}{\mathbf{w}_{:,k}^{(m)^T}} %\mathbf{w}_:k^(m)^T
\DeclareMathOperator{\WkoneT}{\mathbf{w}_{:,k}^{(1)^T}} %\mathbf{w}_:k^(1)^T
\DeclareMathOperator{\WktwoT}{\mathbf{w}_{:,k}^{(2)^T}} %\mathbf{w}_:k^(2)^T
\DeclareMathOperator{\Wdm}{\mathbf{w}_{d,:}^{(m)}} %\mathbf{w}_d:^(m)
\DeclareMathOperator{\Wdone}{\mathbf{w}_{d,:}^{(1)}} %\mathbf{w}_d:^(1)
\DeclareMathOperator{\Wdtwo}{\mathbf{w}_{d,:}^{(2)}} %\mathbf{w}_d:^(2)
\DeclareMathOperator{\WdmT}{\mathbf{w}_{d,:}^{(m)^T}} %\mathbf{w}_d:^(m)^T
\DeclareMathOperator{\WdoneT}{\mathbf{w}_{d,:}^{(1)^T}} %\mathbf{w}_d:^(1)^T
\DeclareMathOperator{\WdtwoT}{\mathbf{w}_{d,:}^{(2)^T}} %\mathbf{w}_d:^(2)^T
\DeclareMathOperator{\Wdkm}{w_{d,k}^{(m)}} %w_dk^(m)
\DeclareMathOperator{\Wdkone}{w_{d,k}^{(1)}} %w_dk^(1)
\DeclareMathOperator{\Wdktwo}{w_{d,k}^{(2)}} %w_dk^(2)
\DeclareMathOperator{\WdkmT}{w_{d,k}^{(m)^T}} %w_dk^(m)^T
\DeclareMathOperator{\WdkoneT}{w_{d,k}^{(1)^T}} %w_dk^(1)^T
\DeclareMathOperator{\WdktwoT}{w_{d,k}^{(1)^T}} %w_dk^(2)^T

\DeclareMathOperator{\Vm}{\mathbf{\tilde{X}}^{(m)}} %V^(m)
\DeclareMathOperator{\VmT}{\mathbf{\tilde{X}}^{(m)^T}} %V^(m)
\DeclareMathOperator{\Vnm}{\mathbf{\tilde{x}}_{\tilde{n},:}^{(m)}} %V_n:^(m)
\DeclareMathOperator{\Vonem}{\mathbf{\tilde{x}}_{1,:}^{(m)}} %V_n:^(m)
\DeclareMathOperator{\VNm}{\mathbf{\tilde{x}}_{\tilde{N},:}^{(m)}} %V_n:^(m)
\DeclareMathOperator{\Vndm}{\tilde{x}_{\tilde{n},d}^{(m)}} %V_n:^(m)
\DeclareMathOperator{\VnmT}{\mathbf{\tilde{x}}_{\tilde{n},:}^{(m)^T}} %V_n:^(m)

\DeclareMathOperator{\bim}{\text{\boldmath$b$}^{(m)}} %alpha^(m)
\DeclareMathOperator{\bidm}{\text{$b$}_d^{(m)}} %alpha^(m)
\DeclareMathOperator{\bimT}{\text{\boldmath$b$}^{(m)^T}} %alpha^(m)

\DeclareMathOperator{\am}{\text{\boldmath$\alpha$}^{(m)}} %alpha^(m)
\DeclareMathOperator{\aone}{\text{\boldmath$\alpha$}} %alpha^(1)
\DeclareMathOperator{\atwo}{\text{\boldmath$\alpha$}^{(2)}} %alpha^(2)
\DeclareMathOperator{\akm}{\alpha_k^{(m)}} %alpha_k^(m)
\DeclareMathOperator{\akone}{\alpha_k} %alpha_k^(1)
\DeclareMathOperator{\aktwo}{\alpha_k^{(2)}} %alpha_k^(2)
\DeclareMathOperator{\akthree}{\alpha_k^{(3)}} %alpha_k^(3)

\DeclareMathOperator{\etam}{\text{\boldmath$\eta^{(m)}$}} %alpha^(m)
\DeclareMathOperator{\etadm}{\text{$\eta_d^{(m)}$}} %alpha^(m)

\DeclareMathOperator{\gamm}{\text{\boldmath$\gamma$}^{(m)}} %gamma^(m)
\DeclareMathOperator{\gamone}{\text{\boldmath$\gamma$}^{(1)}} %gamma^(1)
\DeclareMathOperator{\gamtwo}{\text{\boldmath$\gamma$}^{(2)}} %gamma^(2)
\DeclareMathOperator{\gamdm}{\gamma_d^{(m)}} %gamma_d^(m)
\DeclareMathOperator{\gamum}{\gamma_u^{(m)}} %gamma_d^(m)
\DeclareMathOperator{\gamnm}{\gamma_{n}^{(m)}} %gamma_d^(m)
\DeclareMathOperator{\gamnsm}{\gamma_{\tilde{n}}^{(m)}} %gamma_d^(m)
\DeclareMathOperator{\gamdone}{\gamma_d^{(1)}} %gamma_d^(1)
\DeclareMathOperator{\gamdtwo}{\gamma_d^{(2)}} %gamma_d^(2)

\DeclareMathOperator{\tauo}{\tau^{(O)}} %tau^(a)
\DeclareMathOperator{\taua}{\tau^{(A)}} %tau^(a)
\DeclareMathOperator{\taum}{\tau^{(m)}} %tau^(m)
\DeclareMathOperator{\tauD}{\tau^{(D)}} %tau^(a)
\DeclareMathOperator{\taumt}{\tau^{\{\M_t\}}} %tau^(m)
\DeclareMathOperator{\taummt}{\tau^{(m_t)}} %tau^(m)
\DeclareMathOperator{\taumout}{\tau^{\{\M_{out}\}}} %tau^(m)
\DeclareMathOperator{\tauone}{\tau^{(M)}} %tau^(1)
\DeclareMathOperator{\tautwo}{\tau^{(2)}} %tau^(2)

\DeclareMathOperator{\tm}{\mathbf{T}^{(m)}} %t^(m)
\DeclareMathOperator{\tnm}{\mathbf{t}_{n,:}^{(m)}} %t_n^(m)^*
\DeclareMathOperator{\tnmt}{\mathbf{t}_{n,:}^{\{\M_t\}}} %t_n^(m)^*
\DeclareMathOperator{\tndotm}{\mathbf{t}_{n,:}^{(m)}} %t_n^(m)^*
\DeclareMathOperator{\tndotmt}{t_{n,:}^{\{\M_t\}}} %t_nd^(m_out)
\DeclareMathOperator{\tndotmmt}{t_{n,:}^{(m_t)}} %t_nd^(m_out)
\DeclareMathOperator{\tmss}{\mathbf{T}^{(m_{ss})}} %t^(m_ss)
\DeclareMathOperator{\tmS}{\mathbf{T}^{(m)*}} %t^(m)^(*)
\DeclareMathOperator{\tmssS}{\mathbf{T}^{(m_{ss})*}} %t^(m_ss)^(*)
\DeclareMathOperator{\tmoutS}{\mathbf{T}^{\{\M_{out}\}*}} %t^(m)^(*)
\DeclareMathOperator{\tnmoutS}{\mathbf{t}^{\{\M_{out}\}}_{new,:}} %t^(m)^(*)
\DeclareMathOperator{\tmout}{\mathbf{T}^{\{\M_{out}\}}} %t^(m)^(*)
\DeclareMathOperator{\tmtS}{\mathbf{T}^{\{\M_t\}*}} %t^(m)^(*)
\DeclareMathOperator{\tmt}{\mathbf{T}^{\{\M_t\}}} %t^(m)^(*)
\DeclareMathOperator{\tnmS}{\mathbf{t}_{n,:}^{(m)*}} %t_n^(m)^(*)
\DeclareMathOperator{\tndmS}{t_{n,d}^{(m)*}} %t_nd^(m)^(*)
\DeclareMathOperator{\ttwo}{T} %t^(2)
\DeclareMathOperator{\tthree}{\mathbf{T}^{(3)}} %t^(3)
\DeclareMathOperator{\tntwo}{\mathbf{t}_{n,:}^{(2)}} %t_n^(2)
\DeclareMathOperator{\tndtwo}{t_{n,d}^{(2)}} %t_nd^(2)
\DeclareMathOperator{\ttwoT}{\mathbf{T}^{(2)^T}} %t^(2)^T
\DeclareMathOperator{\ttwoS}{\mathbf{T}^{(2)*}} %t^(2)^*
\DeclareMathOperator{\tntwoS}{\mathbf{t}_{n,:}^{(2)*}} %t^(2)^*
\DeclareMathOperator{\tntwoT}{\mathbf{t}_{n,:}^{(2)^T}} %t_n^(2)^T
\DeclareMathOperator{\tndm}{t_{n,d}} %t_nd^(m)
\DeclareMathOperator{\tn}{t_{n,:}} %t_nd^(m)
\DeclareMathOperator{\dndm}{d_{n,1}} %t_nd^(m)

\DeclareMathOperator{\tndtwoT}{t_{n,d}^{(2)^T}} %t_nd^(2)^T
\DeclareMathOperator{\tndtwoS}{t_{n,d}^{(2)*}} %t_nd^(2)^*
\DeclareMathOperator{\tndmout}{t_{n,d}^{\{\M_{out}\}}} %t_nd^(m_out)
\DeclareMathOperator{\tndmoutT}{t_{n,d}^{\{\M_{out}\}^T}} %t_nd^(m_out)^T
\DeclareMathOperator{\tndmoutS}{t_{new,d}^{\{\M_{out}\}}} %t_nd^(m_out)*
\DeclareMathOperator{\tndt}{t_{n,d}^{\{\M_{t}\}}} %t_nd^(m_out)
\DeclareMathOperator{\tndtT}{t_{n,d}^{\{\M_{t}\}^T}} %t_nd^(m_out)^T
\DeclareMathOperator{\tndtS}{t_{n,d}^{\{\M_{t}\}*}} %t_nd^(m_out)*
\DeclareMathOperator{\tndmss}{t_{n,d}^{\{\M_{ss}\}}} %t_nd^(m_ss)
\DeclareMathOperator{\tndmssS}{t_{n,d}^{\{\M_{ss}\}*}} %t_nd^(m_ss)*

\DeclareMathOperator{\ttm}{\mathbf{t}^{(m)}} %t^(m)
\DeclareMathOperator{\ttmS}{\mathbf{t}^{(m)*}} %t^(m)
\DeclareMathOperator{\ttnm}{t_n^{(m)}} %t^(m)
\DeclareMathOperator{\ttnmS}{t_n^{(m)*  }} %t^(m)
\DeclareMathOperator{\ttnmoutS}{t_{new}^{\{\M_{out}\}}} %t^(m)
\DeclareMathOperator{\ttnmt}{t_{n}^{\{\M_t\}}} %t_n^(m)^*

\DeclareMathOperator{\Ikc}{\mathbf{I}_{K_c}} %t^(m)
\DeclareMathOperator{\Idm}{\mathbf{I}_{D_m}} %t^(m)

\DeclareMathOperator{\sumd}{\sum\limits_{d=1}^{D_m}} %sum_{d=1}^{D_m}
\DeclareMathOperator{\sumdone}{\sum\limits_{d=1}^{D_1}} %sum_{d=1}^{D_1}
\DeclareMathOperator{\sumdtwo}{\sum\limits_{d=1}^{D_2}} %sum_{d=1}^{D_2}
\DeclareMathOperator{\sumn}{\sum\limits_{n=1}^{N}} %sum_{n=1}^{N}
\DeclareMathOperator{\sumns}{\sum\limits_{\tilde{\tilde{n}}=1}^{\tilde{N}}} %sum_{n^*=1}^{N^*}
\DeclareMathOperator{\sumu}{\sum\limits_{u=1}^{N}} %sum_{n^*=1}^{N^*}
\DeclareMathOperator{\summ}{\sum\limits_{m=1}^{M}} %sum_{m=1}^{2}
\DeclareMathOperator{\sumk}{\sum\limits_{k=1}^{K_c}} %sum_{k=1}^{K_c}

\DeclareMathOperator{\prodd}{\prod\limits_{d=1}^{D_m}} %prod_{d=1}^{D_m}
\DeclareMathOperator{\proddone}{\prod\limits_{d=1}^{D_1}} %prod_{d=1}^{D_1}
\DeclareMathOperator{\proddtwo}{\prod\limits_{d=1}^{D_2}} %prod_{d=1}^{D_2}
\DeclareMathOperator{\prodn}{\prod\limits_{n=1}^{N}} %prod_{n=1}^{N}
\DeclareMathOperator{\prodns}{\prod\limits_{\tilde{n}=1}^{\tilde{N}}} %prod_{n=1}^{N}
\DeclareMathOperator{\prodk}{\prod\limits_{k=1}^{K_c}} %prod_{k=1}^{K_c}
\DeclareMathOperator{\prodm}{\prod\limits_{m=1}^{M}} %prod_{m=1}^{2}
\DeclareMathOperator{\produ}{\prod\limits_{u=1}^{N}} %sum_{n^*=1}^{N^*}


% ********************************************************************************* %

\DeclarePairedDelimiter\ang{\langle}{\rangle}
\newcommand{\lnp}[1]{\ln\p*{#1}} %Expectation
\newcommand{\eqline}{\enskip&\enskip}
\newcommand{\eqeq}{\enskip=&\enskip}
\newcommand{\eqapprox}{\enskip\approx&\enskip}
\newcommand{\eqsimil}{\enskip\sim &\enskip}

